Relate and Predict: Structure-Aware Prediction with Jointly Optimized Neural DAG

Understanding relationships between feature variables is one important way humans use to make decisions. However, state-of-the-art deep learning studies either focus on task-agnostic statistical dependency learning or do not model explicit feature dependencies during prediction. We propose a deep neural network framework, dGAP, to learn neural dependency Graph and optimize structure-Aware target Prediction simultaneously. dGAP trains towards a structure self-supervision loss and a target prediction loss jointly. Our method leads to an interpretable model that can disentangle sparse feature relationships, informing the user how relevant dependencies impact the target task. We empirically evaluate dGAP on multiple simulated and real datasets. dGAP is not only more accurate, but can also recover correct dependency structure.

==> 041algo.tex <==
\begin{algorithm}[H]
\SetAlgoLined
\KwResult{Graphs $\boldsymbol{Z}$, Output $\boldsymbol{y}$ }
 initialization\;
 
 $\mathbb{S}(\boldsymbol{x})$
 \caption{\methodName}
\end{algorithm}

==> 0622-dag-old.tex <==

\subsubsection{Real World Dataset: California housing Dataset}
This is a regression data where the target variable is the median house value for California districts. The total number of training points are $20640$.  The number of input features $p=8$. \footnote{The relevant features are median income in block (MedInc), median house age in block (HouseAge), average number of rooms (AveRooms), average number of bedrooms (AveBedrms), block Population, average house occupancy (AveOccup), house block latitude(Latitude) and house block longitude (Longitude).} We scale the features to zero mean and unit variance. We split the data from \cite{pace1997sparse} into train, valid and test using 80/10/10 splits. 
As this is a regression dataset, we learn one graph.  We show the graphs learnt by our method in Figure~\ref{fig:nid_cal} and RMSE~(Root Mean Squared Error) results  in Table~\ref{tab:calhousing}. 

Hyperparameters: We use the validation data to select the best hyperparameters. We use an  initial position embedding $d_{pos}=16$ and $struct_H=16$ with a single layer in the structure learner $\mathcal{S}$.  We vary $task_H$ in the set of $\{16,32,64\}$, $task_L$ in $ \{2,4\}$ and $nheads$ in $ \{4,8\}$. We use dropout of $\{0.3\}$ for the pretraining step in the structure learner $\mathcal{S}$. We use a learning rate of $0.001$ for the Adam Optimizer. We vary $\ell_{sparse}=\{0.001,0.005,0.01\}$. For the MLP baseline, we vary $task_L \in \{2,4,6\}$ and $task_H \in \{16,32,64\}$. We choose the reported based on validation results. 


\paragraph{Qualitative Interpretation:} Figure~\ref{fig:nid_cal}(a) shows that our method is able to successfully learn a relationship between latitude and longitude which is important for house value prediction.  We also show the case where we use solely the task loss to learn a graph in Figure~\ref{fig:nid_cal}(b). While some interactions are similar to (a), without structure loss we cannot recover a strong relationship between latitude and longitude. %





\subsection{Real World Dataset: Heart Disease Prediction Dataset}

We use the Cleveland heart disease dataset from \cite{detrano1986cardiac}.  The task is to predict whether or not a
patient has coronary artery disease given demographic information like age, gender and clinical measurements. After preprocessing,
the dataset contains 298 patients with 13 associated features.
We split the data into training, validation and test  randomly using 70/10/20 splits. 
\vspace{-1mm}
\footnote{The list of features \cite{detrano1986cardiac} are: real variables include: age of patient (age),  resting systolic blood pressure (trestbps), cholesterol (chol), maximum heart rate achieved exercise (thalach) and exercise-induced ST-segment depression (oldpeak). Categorical variables include: type of pain a patient experienced if any (cp), slope of peak exercise ST segment (slope), classification of resting electrocardiogram (restecg), whether or not a patient had thallium defects (thal) as revealed by scintigraphy, number of major vessels appearing to contain calcium as revealed by cinefluoroscopy (ca), gender (gender),whether or not a patient's fasting blood sugar was above 120 mg/dl (fbs),  and whether or not a patient has exercise-induced angina (exang). }
We show the graphs learnt by our method in Figure~\ref{fig:heart} and AUC(Area Under Curve) results obtained in Table~\ref{tab:calhousing}. Our model is able to achieve similar AUC performance along with successfully disentangling dependencies.

Hyperparameters: To select hyperparameters, we use validation AUC for each random seed, and report the test AUC.  We use an  initial position embedding $d_{pos}=16$ and $struct_H=64$ with a single layer in the structure learner $\mathcal{S}$.  We vary $task_H$ in the set of $\{8,16,32\}$, $task_L$ in $ \{2,4\}$ and $nheads$ in $ \{2,4\}$. We use dropout of $\{0.3\}$ for the pretraining step in the structure learner $\mathcal{S}$. We use a learning rate of $0.001$ for the Adam Optimizer. We use $\ell_{sparse}=0.01$ and $\ell_{struct}=1.0$. For the GCN variation, we vary $task_H$ in the set of $\{16,32,64,128\}$, and $task_L$ in $ \{2,4\}$. For the MLP baseline, we vary $task_L \in \{2,4,6\}$ and $task_H \in \{16,32,64\}$. We vary task dropout in $\{0.0,0.1,0.3\}$. We report average results for two random seeds.

\paragraph{Qualitative Interpretation:}  Figure~\ref{fig:heart} shows the graphs learnt by our {\methodName}. We show a stronger link between Maximum Heart Rate (thalach) and Age in healthy class Figure~\ref{fig:heart}(b), whereas a weaker link in heart disease patients Figure~\ref{fig:heart}(c). We show this explicitly in the differential case Figure~\ref{fig:heart}(d). 



\begin{figure*}[tb]
\begin{minipage}{.55\textwidth}
\begin{center}
\setlength\tabcolsep{0.5pt} 
\begin{tabular}{cc}
\includegraphics[scale=0.16]{housing.pdf}&
\includegraphics[scale=0.16]{housing_no_struct_no_sparse.pdf}\\
(a) &  (b) \\
\end{tabular}
\end{center}
\end{minipage}%
\hfill
\begin{minipage}{.44\textwidth}
\caption{
Heatmaps of pairwise interaction strengths learnt by {\methodName}  on the Cal-Housing data: (a) Graph learnt by {\methodName}. Our method is able to successfully learn a relationship between latitude and longitude; (b) Graph learnt by {\methodNameNSparse}. While some interactions are shared with (a), without structure loss we cannot recover  a strong relationship between latitude and longitude. %
\label{fig:nid_cal}
}
\end{minipage}
\end{figure*}


\begin{table*}[ht]
    \centering
    \begin{tabular}{|l|c|c|c|}\hline
       Models, Baselines, Ablation Variations  & Housing (RMSE) & Heart (AUC) & Letter (AUC) \\\hline\hline
       {\methodName}  & \textbf{0.4967}  &  0.8616 & 0.9985\\\hline
       {\methodNameNS} &  0.5040 & 0.8804 & 0.9981\\\hline
       {\methodNameNSparse} &  0.5061 & 0.8643 & 0.9984\\\hline
       {\methodNameGCN} & 0.9155 &  0.8966 &0.7233  \\\hline
       M-{\methodName} & NA & 0.8482 & 0.9983\\\hline
        M-{\methodNameNS} & NA  & 0.8481 & 0.9983 \\\hline
        M-{\methodNameNSparse} & NA & 0.8607  & \textbf{0.9988} \\\hline
        
        M-{\methodNameGCN} & NA & \textbf{0.9016} &  0.7274\\\hline\hline
       GAT-FC & 0.5043 & 0.8692   & \textbf{0.9985}\\\hline
        MLP & \textbf{0.5028} & \textbf{0.8884} &0.9981\\\hline
    \end{tabular}
    \caption{Real Data Results. For Housing Dataset (column 1) we report Root Mean Squared Error (RMSE), For Heart dataset (column 2) and Letter (column 3), we report Area Under Curve (AUC). }
    \label{tab:calhousing}
\end{table*}



\begin{figure*}[tbh]
\begin{center}
\setlength\tabcolsep{0.1pt} 
\begin{tabular}{cccc}
\includegraphics[scale=0.15]{heart_single.pdf}&
\includegraphics[scale=0.15]{heart_0.pdf}&
\includegraphics[scale=0.15]{heart_1.pdf}&
\includegraphics[scale=0.15]{heart_differential.pdf}\\
(a) & (b)  & (c)  & (d) \\
\end{tabular}
\end{center}
\vspace{-0.1in}
\caption{On heart disease data: 
Heatmaps of pairwise interaction strengths learnt by {\methodName} and variations.
(a) The dependency graph learnt by {\methodName}. (b) and (c) Class specific graphs learnt by M-{\methodName}. We show a stronger link between Maximum Heart Rate (thalach) and Age in healthy case (b), whereas a weaker link in disease case (c). We show this differential graph explicitly in (d). %
\label{fig:heart}
}
\end{figure*}




==> 99-050-relatedMore.tex <==
\subsection{Connecting to More General Studies of Data-Driven Discovery of Variable Interactions}

In this section, we briefly discuss the recent related work under the broad area of joint(multi-task) graph structure learning:


 \paragraph{Semi-supervised Link Prediction:}
   A closely related domain within the graph structure learning task is Link Prediction\cite{liben2007link}, where given some part of a network, the task is to find  future or missing links in the rest of the network. This has wide applications in citation, biological and social networks, knowledge bases, etc. Most studies predict links between two nodes in the network based on  heuristic similarity scores, for example, common neighbors, Preferential Attachment\cite{newman2001clustering}, etc. Recent state-of-the-art methods are non-heuristic deep neural network based models\cite{grover2016node2vec,liben2007link,zhang2018link,NIPS2018_7763}. 
     In the context of our work, multiple studies\cite{davis2011multi,ermics2015link} have leveraged evidence from different data sets to predict links representative of multiple conditions, especially in the case of sparsely observed networks. Similarly, \cite{kshirsagar2017multitask,cao2010transfer} formulate it as a multitask matrix completion problem. 
     
     However, in contrast to our work, most of these link prediction methods are inherently semi-supervised, wherein a snapshot of the network is observed. On the other hand, \cite{franceschi2019learning} learns a network in cases where the graph is completely missing, however, it is specific to  node classification tasks using Graph Convolutional Networks. 
     
 \paragraph{Graph Attention Based Interaction Learning in DNNs:}  Graph Attention Networks \cite{velivckovic2017graph} can provide pairwise importance scores for input variable pairs guided by each input's classification objective. Similarly, \cite{yang2018glomo} predict  sample level latent relational graphs that represent dependencies between pairs of data units aimed at transfer learning to downstream tasks.  In contrast, 
our task focuses on learning {\it global} dependency graphs representative of populations, specifically the difference between conditions.

While deep learning based models have shown promise, they do not fit low sample high dimensional regimes. Additionally, these are ``black-box models", that do not provide any insights regarding the logic behind the selection of an edge, which can be important for safety-critical applications like healthcare. 
      
 \paragraph{Graphical Model based:}
        \begin{itemize}
        \item  Undirected Graphical Model based  Estimators : A number of previous work has tried to estimate the differential graph in other data settings, although none of these methods incorporate additional knowledge. \cite{xu2016semiparametric} propose differential estimator for  two semiparametric
elliptical distributions based on quasi likelihood maximization. \cite{zhao2019direct} learns differential functional graphs for applications where data can be regarded as high-dimensional random function vectors. 
            \item Bayesian Networks: Another category of work aims to disentangle  directed relationships between input features. Bayesian networks or Directed Acyclic Graphs are used to represent these dependencies, where the direction of each edge can indicate the direction of causality.  %
        A number of methods focus on learning Bayesian Networks from observational data. %
        These methods can be constraint-based or score-based\cite{koller2009probabilistic}.  More closely relevant to our work, multiple studies \cite{oyen2012leveraging,niculescu2005learning,luis2010inductive} have addressed the problem of estimating Bayesian Networks in a multitask framework.

\item Recently, associating causal mechanisms with Bayesian networks has gained traction. When learning only from observational data, the causal Bayesian networks can only be identified upto a Markov Equivalence Class. To recover the exact causal graph,  a lot of prior work has considered multiple interventional distributions to estimate true causal relationships\cite{cooper1999causal,heckerman1995learning,hauser2012characterization}. 
In contrast to our work, these studies focus on directed networks under intervention distributions, which  can be costly or infeasible. 


        \end{itemize}
      

 \paragraph{Latent Variable Based Graph Estimation:}   Neural Relational Inference\cite{kipf2016variational}, specific to dynamical interacting systems, learns pairwise interactions between input units. This work represents the edges as latent variables in a Variational Autoencoder framework.   While these models can possibly be extended to a differential network estimation using a multitask framework, the former is limited to Graph Convolutional Network based node classification settings. In contrast, while the latter is an unsupervised graph learning framework, it is designed for dynamically interacting input systems, with each system determined by a specific interaction structure. %


 Joint Learning of Graph and Graph Representation Learning: The aforementioned \cite{franceschi2019learning}  learns a probabilistic generative model to represent a network between input nodes guided by a node classification objective.
        
  


==> 99-062-nid-more.tex <==

\begin{figure*}[tbh]
\begin{center}
\setlength\tabcolsep{0.3pt} 
\begin{tabular}{ccc}
\includegraphics[scale=0.20]{letter.png}&
\includegraphics[scale=0.20]{letter_multi_a.pdf}&
\includegraphics[scale=0.20]{letter_multi_b.pdf}\\
(a) SingleGraph & (b) Class A & (c) Class B \\
\end{tabular}
\end{center}
\caption{On Letter Data: 
Heat maps of pairwise interaction strengths learnt by {\methodName} framework on letter dataset. (a) shows the graph learnt by {\methodName}. (b) and (c) shows graphs learnt for each class by M-{dGAP}. Most features are densely connected to each other in the Letter dataset.\label{fig:letter} 
}
\vfill
\end{figure*}


\subsection{Real World Dataset: California Housing Dataset}
The relevant features are median income in block (MedInc), median house age in block (HouseAge), average number of rooms (AveRooms), average number of bedrooms (AveBedrms), block Population, average house occupancy (AveOccup), house block latitude(Latitude) and house block longitude (Longitude).

Hyperparameters: We use the validation data to select the best hyperparameters. We use an  initial position embedding $d_{pos}=16$ and $struct_H=16$ with a single layer in the structure learner $\mathcal{S}$.  We vary $task_H$ in the set of $\{16,32,64\}$, $task_L$ in $ \{2,4\}$ and $nheads$ in $ \{4,8\}$. We use dropout of $\{0.3\}$ for the pretraining step in the structure learner $\mathcal{S}$. We use a learning rate of $0.001$ for the Adam Optimizer. We vary $\ell_{sparse}=\{0.001,0.005,0.01\}$. For the MLP baseline, we vary $task_L \in \{2,4,6\}$ and $task_H \in \{16,32,64\}$. We choose the reported based on validation results. 
\subsection{Real World Dataset : Heart Disease Prediction Dataset}
The list of features, along with their short names in parantheses \cite{detrano1986cardiac} are: real variables include: age of patient (age),  resting systolic blood pressure (trestbps), cholesterol (chol), maximum heart rate achieved exercise (thalach) and exercise-induced ST-segment depression (oldpeak). Categorical variables include: type of pain a patient experienced if any (cp), slope of peak exercise ST segment (slope), classification of resting electrocardiogram (restecg), whether or not a patient had thallium defects (thal) as revealed by scintigraphy, number of major vessels appearing to contain calcium as revealed by cinefluoroscopy (ca), gender (gender),whether or not a patient's fasting blood sugar was above 120 mg/dl (fbs),  and whether or not a patient has exercise-induced angina (exang). 

Hyperparameters: To select hyperparameters, we use validation AUC for each random seed, and report the test AUC.  We use an  initial position embedding $d_{pos}=16$ and $struct_H=64$ with a single layer in the structure learner $\mathcal{S}$.  We vary $task_H$ in the set of $\{8,16,32\}$, $task_L$ in $ \{2,4\}$ and $nheads$ in $ \{2,4\}$. We use dropout of $\{0.3\}$ for the pretraining step in the structure learner $\mathcal{S}$. We use a learning rate of $0.001$ for the Adam Optimizer. We use $\ell_{sparse}=0.01$ and $\ell_{struct}=1.0$. For the GCN variation, we vary $task_H$ in the set of $\{16,32,64,128\}$, and $task_L$ in $ \{2,4\}$. For the MLP baseline, we vary $task_L \in \{2,4,6\}$ and $task_H \in \{16,32,64\}$. We vary task dropout in $\{0.0,0.1,0.3\}$. We report average results for two random seeds.

\subsection{Real World Dataset: Letter Dataset}

The Letter Dataset\cite{frey1991letter} is a  letter recognition
dataset that contains 20k data points of transformed features for binary classification of letters on a pixel
display. The total number of samples are $20k$, with total number of features $16$. We divide into train valid and test into 80,20,20 splits. The binary classification task from the letter dataset is to distinguish letters A-M from N-Z using 16 pixel display features.




We use the validation data to select the best hyperparameters. We use an  initial embedding of $16$ and $struct_H=32$ with a single layer in the structure learner $\mathcal{S}$.  We vary $task_H$ in the set of $\{16,32,64\}$, $task_L$ in $ \{2,4\}$ and $nheads$ in $ \{4,8\}$. We use dropout of $\{0.3\}$ for the pretraining step in the structure learner $\mathcal{S}$. We use a learning rate of $0.001$ for the Adam Optimizer. We vary $\ell_{sparse}=\{0.001,0.005\}$. We report the average over $3$ random seeds. 
 We show the graphs learnt by our method in Figure~\ref{fig:letter} and AUC(Area Under Curve) results obtained in Table 2. Our model is able to achieve similar AUC performance along with successfully disentangling dependencies.
\paragraph{Qualitative Interpretation:} We show that most features are densely connected to each other in the Letter dataset.  This is further supported by the similar classification performance across all settings.




==> math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

